A Method for the Automated Discovery of Angle Theorems

The Naive Angle Method, used by Geometry Expressions for solving problems which involve only angle constraints, represents a geometrical configuration as a sparse linear system. Linear systems with the same underlying matrix structure underpin a number of different geometrical theorems. We use a graph theoretical approach to define a generalization of the matrix structure.

==> eptcsdata.tex <==
\providecommand{\firstpage}{148}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.17}{10.4204/EPTCS.352.17}}

